Modeling Content and Context with Deep Relational Learning

Building models for realistic natural language tasks requires dealing with long texts and accounting for complicated structural dependencies. Neural-symbolic representations have emerged as a way to combine the reasoning capabilities of symbolic methods, with the expressiveness of neural networks. However, most of the existing frameworks for combining neural and symbolic representations have been designed for classic relational learning tasks that work over a universe of symbolic entities and relations. In this paper, we present DRaiL, an open-source declarative framework for specifying deep relational models, designed to support a variety of NLP scenarios. Our framework supports easy integration with expressive language encoders, and provides an interface to study the interactions between representation, inference and learning.

==> 6modeling.tex <==
\section{Modeling Strategies}\label{sec:modeling}
%
\ml{TO-DO: Update this section}

\noindent\textbf{(1) Embed Symbol / Explain Data} This representation learning objective aligns the embedding of symbolic entities and raw entities, grounding the symbol in the raw data, and using the symbol embedding to explain properties of previously unseen raw-entity instances. For example, consider the rule: {\small$\mathtt{Issue(T, I)} \wedge \mathtt{InThread(T, P)} \Rightarrow \mathtt{Pro(P, I)}$}. Issue (I) is a symbolic entity representing a debate topic (e.g. gun-control), and post (P) is a raw entity representing the debate post content. The $\mathtt{Pro}$ relation defines the positive and negative examples for the representation learning objective. This way, the embedding of issues and posts that support them will be closer in the embedding space.%for a given thread, and likewise, the embeddings of issues and posts that oppose them will be distant in the embedding space. 

%\paragraph{Explain} This is the analogous case to the \textit{embed symbol} objective, where we map raw entities to symbolic entities. Consider the same rule as above, where issues and posts that support them are closer in the embedding space. This results in an embedding for raw entity P that closely aligns with the symbolic issues that they support. 

\noindent\textbf{(2) Translate} This objective aligns the representation of pairs of different symbolic or raw entity types. For example, consider the \DRAIL rule: {\small $\mathtt{InThread(T, U)} \wedge \mathtt{InThread(T, P)} \Rightarrow \mathtt{Author(U, P)}$ }. The representation of the two raw entities, post (P) and user (U), are aligned using the $\mathtt{Author}$ relationship. This way, user information is aligned with textual representation and the vice-versa. Similarly, when defined over pairs of symbolic entities, the correlation between symbols can be captured in the embedding space.

Representation learning can be done end-to-end, as a byproduct of the structured learning objective (Sec. \ref{sec:learning}), or by explicitly defining separate embedding objectives.% Then, learning can be done either simultaneously or as a pre-training step.  



%Optionally, we allow relational encoders to also maintain a set of private, rule-specific, parameters. This is done to prevent a particular rule from hijacking the decision, and allow each rule to be able adapt to task-specific behaviors. 

%\ml{TO-DO: Define entity encoders and add the discussion on embedding objectives embed, translate, explain....}



==> figs/inference_impact_training.tex <==
\begin{tikzpicture}
    \begin{axis}[
        /pgf/number format/.cd,
        1000 sep={},
        width=1\textwidth,
        height=.5\textwidth,
        major x tick style=transparent,
        ybar=7pt,
        bar width=15pt,
        ymajorgrids=true,
        ylabel={Proportion of Training Time},
        label style={font=\Large},
        tick label style={font=\Large},
        symbolic x coords={AM, 4F, OD},
        xticklabels={Argument Mining (BiLSTMs), Stance Prediction (BERT), Open Domain (BERT-small)},
        x tick label style={text width=10em, align=center},
        xtick=data,
        scaled y ticks=false,
        enlarge x limits=0.1,
        ymin=0,
        ymax=16,
        point meta=rawy,
        log ticks with fixed point,
        log origin=infty,
        legend cell align=left,
        nodes near coords,
        every node near coord/.append style={font=\Large, color=black},
        legend columns=2,
        legend style={
                style={font=\Large},
                at={(0.27,0.84)},
                anchor=south west,
                /tikz/column 2/.style={column sep=3ex, font=\Large}
        }
    ]
        % ILP
        \addplot[style={one,fill=one,mark=none}]
            coordinates {(AM, 13.0)(4F, 3.3)(OD, 6.9)};
            
        % AD3
        \addplot[style={two,fill=two,mark=none}]
            coordinates {(AM, 13.3)(4F, 8.9)(OD, 1)};
            
        \legend{DRaiL-ILP, DRaiL-AD$^3$}
    \end{axis}
\end{tikzpicture}

==> figs/inference_runtime.tex <==
\begin{tikzpicture}
    \begin{axis}[
        /pgf/number format/.cd,
        1000 sep={},
        width=1\textwidth,
        height=.5\textwidth,
        major x tick style=transparent,
        ybar=7pt,
        bar width=15pt,
        ymajorgrids=true,
        ylabel={Inference in Seconds},
        label style={font=\Large},
        tick label style={font=\Large},
        symbolic x coords={AM, 4F, OD},
        xticklabels={Argument Mining, Stance Prediction, Open Domain},
        x tick label style={text width=10em, align=center},
        xtick=data,
        scaled y ticks=false,
        enlarge x limits=0.1,
        ymin=0,
        ymax=55,
        point meta=rawy,
        log ticks with fixed point,
        log origin=infty,
        legend cell align=left,
        nodes near coords,
        every node near coord/.append style={font=\normalsize, color=black},
        legend columns=2,
        legend style={
                style={font=\Large},
                at={(0.27,0.84)},
                anchor=south west,
                /tikz/column 2/.style={column sep=3ex, font=\Large}
        }
    ]
        % ILP
        \addplot[style={one,fill=one,mark=none}]
            coordinates {(AM, 17.8)(4F, 5.5)(OD, 45)};

        % AD3
        \addplot[style={two,fill=two,mark=none}]
            coordinates {(AM, 18.3) (4F, 17.5)(OD, 48)};

        % PSL
       % \addplot[style={two,fill=two,mark=none}]
        %     coordinates {(AM, 1) (4F, 1) (OD, 1)};

        \legend{ILP, AD$^3$, PSL}
    \end{axis}
\end{tikzpicture}
